Collaborative Design and Planning of Software Architecture Changes via Software City Visualization

Developers usually use diagrams and source code to jointly discuss and plan software architecture changes. With this poster, we present our on-going work on a novel approach that enables developers to collaboratively use software city visualization to design and plan software architecture changes.

==> chapters/related-work.tex <==
\section{Related Work}\label{sec:related-work}

Todo and test cite~\cite{anslow2013}.
